Sentence-level Online Handwritten Chinese Character Recognition

Single online handwritten Chinese character recognition~(single OLHCCR) has achieved prominent performance. However, in real application scenarios, users always write multiple Chinese characters to form one complete sentence and the contextual information within these characters holds the significant potential to improve the accuracy, robustness and efficiency of sentence-level OLHCCR. In this work, we first propose a simple and straightforward end-to-end network, namely vanilla compositional network~(VCN) to tackle the sentence-level OLHCCR. It couples convolutional neural network with sequence modeling architecture to exploit the handwritten character's previous contextual information. Although VCN performs much better than the state-of-the-art single OLHCCR model, it exposes high fragility when confronting with not well written characters such as sloppy writing, missing or broken strokes. To improve the robustness of sentence-level OLHCCR, we further propose a novel deep spatial-temporal fusion network~(DSTFN). It utilizes a pre-trained autoregresssive framework as the backbone component, which projects each Chinese character into word embeddings, and integrates the spatial glyph features of handwritten characters and their contextual information multiple times at multi-layer fusion module. We also construct a large-scale sentence-level handwriting dataset, named as CSOHD to evaluate models. Extensive experiment results demonstrate that DSTFN achieves the state-of-the-art performance, which presents strong robustness compared with VCN and exiting single OLHCCR models. The in-depth empirical analysis and case studies indicate that DSTFN can significantly improve the efficiency of handwriting input, with the handwritten Chinese character with incomplete strokes being recognized precisely.

==> problem_formulation.tex <==
\section{Problem Formulation}
In this section, we concretely introduce the overview of OLHCCRS task in Section~\ref{3.1} and the mathematical definition in Section~\ref{3.2}.

\subsection{Task Overview}
\label{3.1}
The current single handwritten Chinese character recognition has shown remarkable progress, yet the application scenario of handwritten Chinese character recognition is generally at the sentence level, which confronts the intrinsic difficulty of inferior handwriting recognition efficiency compared to the sentence-level pinyin input method~\cite{pinyin}. To explore efficient sentence-level handwriting input method, we propose the online handwritten Chinese character recognition on sentence-level~(OLHCCRS), where each sample is the sequential handwritten Chinese characters as shown in Figure~\ref{sub.2}. To simulate the sentence-level handwriting input environment, we collect millions of sentences from large news corpus and hundreds of handwritten sets of Chinese characters, which are will introduced in Section~\ref{data_p}. For any handwriting sentence, we further believe that the semantic information of sentences and dependency relationship between words are crucial for promoting the recognition accuracy on sentence-level. 

On the other hand, Chinese characters are composed of multiple strokes. Online handwritten Chinese characters involve digital pens or stylus, where we should constantly obtain the representation of each handwritten character with multiple strokes and real-time predict it. Although the shape of human handwriting generally is changeable even for the same character, the habits of handwriting strokes and language expression are regular. Under the deliberation, we believe that models can quickly and precisely recognise Chinese characters with missing strokes by continuously learning the various patterns of human sentence-level handwritten Chinese characters. If the online handwritten Chinese characters with missing strokes are still recognized with high accuracy, it is a feasible way to improve the recognition efficiency of online sentence-level handwriting Chinese characters. The concrete methods are shown in Section~\ref{sec_sp} and \ref{sec_dstfrn}. To summarise, our proposed OLHCCRS task intends to explore the fast recognition method of handwriting Chinese characters on sentence-level and includes three challenges: 1) the real-time representation of handwritten characters. 2) how to capture the dependency relationship between words. 3) the efficiency and robustness of the designed model.

\subsection{Task Definition}
\label{3.2}

As shown in Figure~\ref{sub.2}, one online handwritten Chinese sentence~(OLHCS) can be denoted as $S=(w_1,..., w_i,..., w_n)$, where $w_i$ represents the $i$th handwritten character in the sentence. Each handwritten Chinese character $w_i$ is composed of multiple strokes, denoted as $w_i=(s_1, s_2,..., s_k)$, where $s_k$ represents the $k$th stroke of $w_i$. For OLHCS, the handwriting sentence is composed of a series of continuous strokes respectively, so we define the sequence of handwritten Chinese characters as $S=(w_{1,1}, ...,w_{1,k_{1}},..., w_{i,j},..., w_{n,k_{n}})$, where $w_{i,j}$ represents the $j$th stroke of the $i$th handwritten character. Despite writers do not necessarily write Chinese characters in the correct order of strokes, each handwritten character sample can be divided into multiple fragments~(at least the whole character) according to the handwriting pattern of humans. The inputs of our task include the sequential strokes of handwritten characters $S$ and the output is the standard  Chinese characters denoted as $\tilde{S}=(\tilde{w}_{1},...,\tilde{w}_{n})$, where $\tilde{w}_{i}$ represents the $i$th word in the sentence.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.95\textwidth]{2.eps}
    \caption{The overall architecture of SRDCNN-GPT, composed of  SRDCNN and GPT-2. The number N is set to 4.}
    \label{fig:model_1}
\end{figure*}
%\noindent\textbf{Data Preprocessing} We 
